Kantian Deontology Meets AI Alignment: Towards Morally Grounded Fairness Metrics

Deontological ethics, specifically understood through Immanuel Kant, provides a moral framework that emphasizes the importance of duties and principles, rather than the consequences of action. Understanding that despite the prominence of deontology, it is currently an overlooked approach in fairness metrics, this paper explores the compatibility of a Kantian deontological framework in fairness metrics, part of the AI alignment field. We revisit Kant's critique of utilitarianism, which is the primary approach in AI fairness metrics and argue that fairness principles should align with the Kantian deontological framework. By integrating Kantian ethics into AI alignment, we not only bring in a widely-accepted prominent moral theory but also strive for a more morally grounded AI landscape that better balances outcomes and procedures in pursuit of fairness and justice.

==> content/mysc.tex <==
\carlos{dictated from emily's work}
Executive orders and other regulatory framework disparate measurements and bias mitigation is called for both in government and in many application areas such as employment, housing, credit, healthcare, criminal just along other including private industry.

This executive orders are asking for various agencies such has the department of labor... to produce their own guidelines... on how algorithmic systems.... 

All the EO is telling things for the government to do, and having impact of private industry. 


What different about this new mandates, its illegal to discriminate in many areas using any decision making systems. It has not been entirely clear how existing discrimination law applies to algorithmic systems. 

Whether an AI system is acting in a discriminatory action. This 

What are the legal doctrines that we have available to measure or mitigate discrimination?

Disparate treatment doctricen, title 7 of the civil rights act, housing act, equal credit act. DT doctrine says that you cant intentionally discraminte against any discriminate group such as ....
The way that this si interpreted in AI system, is that you cant use PT information in your model to influence its prediction or decision. You cant use Race as input. Even if you don't use the prott attribute there are still features that can correlate or contain information about the protected attribute, 

Disparatement impact doctrine, it does not look at the intentions of the organization when using AI decision systems. But instead the DI doctrine, an AI model can not have different protected groups unless they can prove that is necessary for the business -- there is no number to measure DI--. 

DI Three step process.Actors are the organization with the model, and the plaintiff the institution arguien that there is discrimination

1. Shows that there is a difference across prott att. 

2. The defendant claim that there is a business necessity for this decision making system.s

3. If there can be a less discriminatory algorithm than  satisfy the business necessity. 

\carlos{end dictation}
%\subsection{Generative AI for Customized Educational Content}

%In the case of an education and technology company, that specializes in creating personalized educational content for students \enquote{EdGenAI}. The aim is to use generative AI systems which can produce customized learning materials based on individual student profiles. These profiles are created using data such as learning styles, interests, academic strengths and weaknesses, and other personal preferences~\citep{kasneci2023chatgpt}. The challenge from a deontological ethics perspective relies on:


%\paragraph{The Issue of Aggregation.} Ensuring that the AI systems respects the intrinsic worth of each student, treating them not merely as data points but as individuals with unique learning needs and preferences. The AI system should be designed to recognize and respect the unique educational needs and preferences of each student and not seggregating by non choosen factors at birth, this means moving beyond one-size-fits-all content to truly personalized learning experiences that consider the whole student - their interests, cultural background, learning pace, and more.

%\paragraph{Utilitarian Metrics and Deontological Alignment.} To evaluate the performance of and education and generative AI, one might propose metrics such as learning improvements, engagement levels, or user satisfaction. However, in alignment with Kantian deontology, we argue that these metrics should focus on the inherent qualities of the content produced, rather than solely on the outcomes or utility derived from the content. From a deontological perspective, it is the nature and integrity of the educational content that hold paramount importance. Therefore, metrics assessing the fidelity of the AI-generated content to established educational standards, textbook knowledge, and institutional curriculum alignment are of interest if aiming to aling with Kantian deontological principle. These metrics ensure that the EduGenAI system adheres to the ethical deontological principles. For example, an algorithm that optimizes student engagement by generating hallucination or content that has low fidelity to text book knowledge will be considered deontologically unethical even if it achieves optimal engagement metrics.

%\paragraph{No Trade-off Between Fairness and Performance}

%\paragraph{Procedural Fairness.} Aligning with  Kantian emphasis on procedural ethics, the process of how the generative AI system produces content is as important as the decision itself. Therefore, we can not say that a generative AI education system is ethical if the whole pipeline does not ethical standards in each step. This may include \carlos{\ldots}
